Detection of Fights in Videos: A Comparison Study of Anomaly Detection and Action Recognition

Detection of fights is an important surveillance application in videos. Most existing methods use supervised binary action recognition. Since frame-level annotations are very hard to get for anomaly detection, weakly supervised learning using multiple instance learning is widely used. This paper explores the detection of fights in videos as one special type of anomaly detection and as binary action recognition. We use the UBI-Fight and NTU-CCTV-Fight datasets for most of the study since they have frame-level annotations. We find that the anomaly detection has similar or even better performance than the action recognition. Furthermore, we study to use anomaly detection as a toolbox to generate training datasets for action recognition in an iterative way conditioned on the performance of the anomaly detection. Experiment results should show that we achieve state-of-the-art performance on three fight detection datasets.

==> backup.tex <==
The basic cross-entropy loss function is most commonly used. For the action recognition of fights, it becomes the binary cross entropy function, 
\begin{equation}
    L_{BCE}( = 1/N {\sum_{i=1}^N y_ilog(p(y_i) + (1-y_i) log(1-p(y_i))}
\label{eq1}
\end{equation}
where $y$ is the label and $p(y)$ is the predicted probability of y for all N points.

